Mixed-Precision in High-Order Methods: the Impact of Floating-Point Precision on the ADER-DG Algorithm

We present a mixed-precision implementation of the high-order discontinuous Galerkin method with ADER time stepping (ADER-DG) for solving hyperbolic systems of partial differential equations (PDEs) in the hyperbolic PDE engine ExaHyPE. The implementation provides a simple API extension for specifying the numerical precision for individual kernels, and thus allows for testing the effect of low and mixed precision on the accuracy of the solution. To showcase this, we study the impact of precision on the overall convergence order and actual accuracy of the method as achieved for four common hyperbolic PDE systems and five relevant scenarios that feature an analytic solution. For all scenarios, we also assess how sensitive each kernel of the ADER-DG algorithm is to using double, single or even half precision. This addresses the question where thoughtful adoption of mixed precision can mitigate hurtful effects of low precision on the overall simulation.

==> chapters/ADER.tex <==
\section{The ADER-DG method}\label{chapter:ader}

ExaHyPE \cite{Reinarz_ExaHyPE_2020} solves hyperbolic systems of PDEs, which it expects to be expressed in the following canonical form:
%
\begin{equation}\label{eq:exa_canonical_form}
    \frac{\partial Q}{\partial t} + \nabla \cdot F(Q, \nabla Q) + B(Q) \cdot \nabla Q = S(Q) + \sum_{i = 1}^{n_\text{ps}} \delta_i 
\end{equation}
%
where $Q$ is the state vector of quantities. $F$ defines the conservative part and $B$ defines the non-conservative part of the flux. Source terms are expressed in $S$, and $\delta_i$ can be used to specify $n_\text{ps}$ different point sources. 
ExaHyPE2, the latest version of ExaHyPE, relies on Peano4 \cite{Weinzierl:2019:Peano} as mesh infrastructure, which provides dynamically adaptive Cartesian meshes which are efficiently traversed using a spacetree method parallelized by MPI+OpenMP.

The ADER-DG method (Discontinuous Galerkin with Arbitrary high-order DERivative time stepping), as introduced by Dumbser et al.~\cite{dumbser_ader_2014}, is the main numerical approach used in ExaHyPE and also the solver used throughout this work. 
Particularly for non-linear problems, the ADER-DG solver can be complemented with an a-posteriori subcell Finite Volume limiter, whereby unphysical or oscillatory solutions are detected and solutions in respective elements are recomputed with a more robust finite volume scheme on a fine subgrid \cite{Zanotti_pos_lim}. 
In this work, however, we will restrict the discussion to scenarios that do not require limiting.-

In the following, we will shortly recapitulate the key steps of the ADER-DG scheme (see \cite{dumbser_ader_2014,Reinarz_ExaHyPE_2020} for further details). 
For simplicity, we restrict this summary to using only conservative fluxes $F(Q)$, i.e., for solving the simplified problem $\frac{\partial Q}{\partial t} + \nabla \cdot F(Q) = 0$ over a spatial domain $\Omega$ and for $t \in [t_\text{start}, t_\text{end}]$. 

ADER-DG starts from the integral over the time step of the weak form of this system of PDEs in space. Considering a single element $\Omega^{(e)}$ and time step, i.e., the domain $\Omega^{(e)}\times [t_0,t_0+\tau]$ (we will use as short notation $\Delta_t := [t_0,t_0+\tau]$). 
Hence, with test functions $\phi_k(x)$ we formulate the weak form in space as 
\begin{equation}\label{eq:integrated_weak_form}
    \int_{\Delta_t} \int_{\Omega^{(e)}} \phi_k(x) \frac{\partial Q(x)}{\partial t} + \phi_k(x) \nabla \cdot F(Q) \ dx \ dt = 0.
\end{equation}

\begin{comment}
We then integrate the first term in \eqref{eq:integrated_weak_form} by parts in time to obtain

\begin{equation}\label{eq:weak_form_2}
    \int_{\Omega_e} \phi_k(x, t_0+\tau) q_h \ dx - \int_{\Omega_e} \phi_k(x, t_0) u_h \ dx - \int_{\Delta_t} \int_{\Omega_e} \frac{\partial \phi_k}{\partial x} q_h \ dx \ dt + \int_{\Delta_t} \int_{\Omega_e} \phi_k(x,t) \nabla \cdot F_h \ dx \ dt = 0
\end{equation}

Then, we replace the solution $Q$ and the fluxes $F(Q)$ by a discrete representation in the space of test functions $\phi(x,t)$:

\begin{equation}
    \begin{aligned}
        q_h = q_h(x,t) = \phi_l \hat{q_l} \\
        F_h = F_h(x,t) = \phi_l \hat{F_l} 
    \end{aligned}
\end{equation}

The chosen basis for the functions $\phi(x,t)$ is a tensor product of Lagrange interpolation polynomials using Gauss-Legendre quadrature points as nodes, i.e. $\phi(x,t) = \sum_{k=0}^N \phi_k(x) * \sum_{l=0}^N \phi_l(t)$. With this choice of basis, the degrees of freedom for the fluxes can be obtained by evaluating the physical fluxes:%, and the initial degrees of freedom for the solution are the solutions at time $t_0$:

\begin{equation}
    \begin{aligned}
%        q_h^0 = q_h(x,t_0) = \phi_l \hat{q_l} \\
        \hat{F_l} = F(\hat{q_l})
    \end{aligned}
\end{equation}

Inserting this representation into \eqref{eq:weak_form_2} and obtain:

\begin{equation}\label{eq:weak_form_2}
    (\int_{\Omega_e} \phi_k(x, t_0+\tau) \phi_l(x, t_0+\tau\ dx - \int_{\Delta_t} \int_{\Omega_e} \frac{\partial \phi_k}{\partial x} \phi_l \ dx \ dt ) \ \hat{q_l} = \int_{\Omega_e} \phi_k(x, t_0) \phi_l \ dx \ \hat{u_l}  - \int_{\Delta_t} \int_{\Omega_e} \phi_k(x,t) \nabla \cdot \phi_l \ dx \ dt \ F(\hat{q_l})
\end{equation}
\end{comment}

Using the product rule for $\nabla \cdot F(Q)$ and the divergence theorem yields the following formulation:
%
\begin{equation}\label{eq:separated_weak_form}
    \int_{\Delta_t} \int_{\Omega^{(e)}} \phi_k(x) \frac{\partial Q(x)}{\partial t} \ dx \ dt + \int_{\Delta_t} \oint_{\partial {\Omega^{(e)}}} \phi_k(x) F(Q)  \ ds \ dt - \int_{\Delta_t} \int_{\Omega^{(e)}} \phi_k(x) \nabla \cdot F(Q) \ dx \ dt = 0.
\end{equation}
%
Finally, we approximate the solution $Q$ in the first term to the space of test functions $\phi(x)$, such that $Q(x,t^n) \approx \phi_l(x) u_l^n$ and then integrate this first term by parts in time: 
%
\begin{equation}\label{eq_weak_form_volume_surface}
    \int_{\Omega^{(e)}} \phi_k(x) \phi_l(x) \ dx \ (u_l^{n+1}-u_l^{n}) = \underbrace{ \int_{\Delta_t} \int_{\Omega^{(e)}} F(q_k) \nabla \cdot \phi_k \ dx \ dt}_{\textbf{volume integral}} - \underbrace{ \int_{\Delta_t} \oint_{\partial \Omega^{(e)}} F(q_k) \phi_k(x) \ ds \ dt }_{\textbf{surface integral}}
\end{equation}
%                       

%Using Lagrange polynomials, the initial values $q_l^0$ can easily be evaluated as $q_l^0=Q(x_l, t_0)$. Gaussian quadrature nodes are used for the support points of the Lagrange polynomial because they allow the approximation of the integral of a given function $f$ over the interval $[a,b]$ by:
%
% \begin{equation}\label{eq:gaussian_quadrature}
%     \int_a^b f(x) \: dx \approx (b-a) \sum_i w_i f((b-a) \xi_i+(b+a))
% \end{equation}
% %
% this approximation is exact for polynomials up to order $2n-1$ when using Gauss-Legendre polynomials, where $n$ is the number of quadrature points used. This means that if they are used as support points for a Lagrange polynomial of order $n-1$, this integration will always be exact for these polynomials, though not necessarily for the underlying function which these polynomials serve to approximate.
% %


\subsection{Predictor}\label{subseq:predictor}

As mentioned, solving equation \eqref{eq_weak_form_volume_surface} requires an element-local spacetime predictor solution $q_l$. Computing it essentially corresponds to a fixed-point problem and can therefore be solved a number of different ways. To illustrate this, one can return to \eqref{eq:exa_canonical_form}, and take its weak form in both space and time:
%
\begin{equation}
    \int_{\Delta_t} \int_{\Omega^{(e)}} \phi_k(x, t) \frac{\partial Q(x)}{\partial t} + \phi_k(x, t) \nabla \cdot F(Q) \ dx \ dt = 0.
\end{equation}
%
Here we ignore the surface integral, which will be solved in the following corrector step, and approximate both the solution and the fluxes in the space of space-time test functions: $q_k(x,t) := \phi_k(x,t) \hat{q_k}$  and $F_k := \phi_k(x,t) \hat{F_k}$. The degrees of freedom $\hat{F_K}$ can be obtained by evaluating the flux function as $\hat{F_k} = F(q_k(x,t))$. This yields:
%
\begin{equation}
    \int_{\Delta_t} \int_{\Omega^{(e)}} \phi_k \hat{q_k} \frac{\partial \phi_l}{\partial t} + \phi_k \hat{F_k} \nabla \cdot \phi_l \ dx dt = 0.
\end{equation}
%
which, since $\hat{q_k}$ and $\hat{F_k}$ are degrees of freedom, can be reformulated as:
\begin{equation}\label{eq:predictor_degrees_of_freedom}
    \int_{\Delta_t} \int_{\Omega^{(e)}} \phi_k  \frac{\partial \phi_l}{\partial t} dx dt \ \hat{q_k} 
    + \int_{\Delta_t} \int_{\Omega^{(e)}} \phi_k \nabla \cdot \phi_l \ dx dt \ \hat{F_k} = 0.
\end{equation}
%
As both of the integral terms contain only the test functions, these can be precomputed over a reference element and adapted to the corresponding physical element using a change of interval. Fluxes are, as mentioned, simply evaluated as the physical fluxes at the respective degrees of freedom. Therefore all that remains is a scheme of the form $K_t \hat{q_k} + K_x F(\hat{q_k}) = 0$, which can be solved using an iterative method \cite{dumbser_2008}.
%
In ExaHyPE this is done in the general case via Picard-iterations following a method developed by Dumbser et al.~\cite{Dumbser2008FiniteVS}. For linear PDEs, ExaHyPE additionally provides a second method using a Cauchy-Kowalevskaya method~\cite{Gassner2011ExplicitOT} which has the benefit of being much more efficient. This gives the $n$-th time-derivative of Q as:
%
\begin{equation}
    \frac{\partial^n Q}{\partial t^n} = (-1)^n (\nabla F)^n Q
\end{equation}
%
these time-derivatives can then be developed into a Taylor series in time of $Q$. Truncating this Taylor series to a given order then produces an approximate solution.

However it is computed, the approximate solution can be used to compute the volume integral term of \eqref{eq_weak_form_volume_surface}. In addition, the predictor computes the projection of the approximate solutions and its fluxes to each face of the cell, which will be used in the corrector to approximate fluxes between neighbouring cells and thereby the surface integral term of \eqref{eq_weak_form_volume_surface}.

\subsection{Corrector}\label{subseq:corrector}

In a second step, the projected values and fluxes from two adjacent cells are used to compute a numerical flux between them at their interface. These projections, as indicated in \ref{subseq:predictor}, use the predictor solution $q_l$ as well. Once the predictor solutions and fluxes $q_k(x,t) := \phi_k(x,t) \hat{q_k}$  and $F_k := \phi_k(x,t) \hat{F_k}$ have been computed, their projections to a given cell boundary can easily be calculated by evaluating the test functions at that cell boundary:

\begin{equation}
\begin{aligned}
    q_k(x_f, t) = \hat{q_k} \phi_k(x_f, t) \\
    F_k(x_f, t) = \hat{F_k} \phi_k(x_f, t) 
\end{aligned}    
\end{equation}

The term $\phi_l(x_f, t)$ for any given face can, similarly to the integral terms in \eqref{eq:predictor_degrees_of_freedom} be precomputed for a reference element, sparing the need for potentially expensive function evaluations.
%
There will therefore be two extrapolated states $q_k^-, F_k^-$ and $q_k^+, F_k^+$ for any given boundary between two neighbouring cells. In order to compute the surface integral we require a flux across this boundary which takes into account the discontinuity between these states. This corresponds to a Riemann problem and, in ExaHyPE, it is per default solved using the so-called local-Lax-Friedrich or Rusanov flux \eqref{eq:rusanov_flux}, though other Riemann solvers can be specified by the user.
%
\begin{equation}\label{eq:rusanov_flux}
    F_\text{Rus} = \frac{1}{2} (F_\text{L} + F_\text{R}) +  \frac{\lambda_{max L,R}}{2} (Q_L - Q_R)
\end{equation}
%
These computed Riemann fluxes can then be integrated over the faces to compute the surface integral term of \eqref{eq_weak_form_volume_surface}, i.e.:
%
\begin{equation}
    \int_{\Delta_t} \oint_{\partial \Omega^{(e)}} F(q_l) \phi_k(x) \ ds \ dt \approx \int_{\Delta_t} \oint_{\partial \Omega^{(e)}} F_\text{Rus}(q_l^-, q_l^+, F_l^-, F_l^+) \phi_l(x) \ ds \ dt 
\end{equation}
%
Where $q_l^-$, $F_l^-$, $q_l^+$, $F_l^+$ are the projections of the predictor solutions and fluxes to the respective surface by the cells on the negative and positive sides of said face respectively.

Finally, we need to compute an appropriate timestep size for the next timestep, stable timestep sizes in the ExaHyPE ADER-DG kernels are computed with a version of the the so-called Courant-Friedrichs-Lewy (CFL) condition~\cite{dumbser_2008}.
%
\begin{equation}\label{eq::CFL_condition}
    \Delta t = \frac{C_\text{CFL} \ dx}{d \ (2N+1) \ \lambda_{max}}
\end{equation}
%
where $C_\text{CFL}$ is a stability factor depending on the polynomial order $N$, $d$ is the number of dimensions of the problem, $dx$ is the size of the cell and $\lambda_{max}$ is the greatest eigenvalue in the cell.

% \subsubsection{Algorithm}
%\newpage
Algorithm \ref{alg:ader} summarizes one step of the ADER-DG algorithm.
%Note that for the sake of performance, the Riemann solvers only get performed once on shared faces instead of being performed once per adjacent cell.

\begin{algorithm}
\caption{The ADER-DG algorithm}\label{alg:ader}
\begin{algorithmic}[1]
\For {cell C in K}
    \State $ (q_t, f(q_t)) \gets \text{spaceTimePredictor}(q_C)$ %\Comment{computed via Picard iteration or CK-method}
    \State $ (\partial q_C, \partial f_C) \gets \text{expansion}(q_t, f(q_t))$ \hspace{1.3em}
        \rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\\{}\\{}\end{array}\color{black}\right\}%
          \color{black}\begin{tabular}{l}Predictor step, combined into the kernel \\ \textbf{fusedSpaceTimePredictorVolumeIntegral()}\end{tabular}$}}
    \State $ q_C += \text{volumeIntegral}(\partial f_C))$
\EndFor
\State $\Delta t_{next} \gets 0$
\For {cell C in K}
    \For {face F  in $\partial K$}
        \State $ flux \gets \textbf{riemannSolver(}(q_{F, left}, q_{F, right}, f_{F, left}, f_{F, right})$
            \rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\\{}\\{}\end{array}\color{black}\right\}%
              \color{black}\begin{tabular}{l}Corrector step\end{tabular}$}}
        \State $ q_{C} += \textbf{faceIntegral}(flux)$
    \EndFor
    \State $\Delta t_{next} \gets \max(\Delta t_{next}, \textbf{computeTimestep}(q_C))$
\EndFor
\end{algorithmic}
\end{algorithm}

==> figures/adaptive_precision/old/HHS_bf16.tex <==
\begin{figure}[ht!]
    \centering
    
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vx,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vx,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vx,x=t]{figures/adaptive_precision/HHS_bf16.dat};
            \addlegendentry{bf16}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vx,
            ymin=-40,
            ymax=40,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vy,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vy,x=t]{figures/adaptive_precision/HHS_bf16.dat};
            \addlegendentry{bf16}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vz,
            ymin=-40,
            ymax=40,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vz,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vz,x=t]{figures/adaptive_precision/HHS_bf16.dat};
            \addlegendentry{bf16}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \caption{TODO, but this is bf16}
\end{figure}

==> figures/adaptive_precision/old/HHS_fp64.tex <==
\begin{figure}[ht!]
    \centering
    
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vx,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vx,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vx,x=t]{figures/adaptive_precision/HHS_fp64.dat};
            \addlegendentry{fp64}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vx,
            ymin=-40,
            ymax=40,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vy,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vy,x=t]{figures/adaptive_precision/HHS_fp64.dat};
            \addlegendentry{fp64}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vz,
            ymin=-40,
            ymax=40,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vz,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vz,x=t]{figures/adaptive_precision/HHS_fp64.dat};
            \addlegendentry{fp64}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \caption{TODO, but this is fp64}
\end{figure}

==> figures/adaptive_precision/old/HHS_mixed.tex <==

\begin{figure}[ht!]
    \centering
    
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vx,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vx,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vx,x=t]{figures/adaptive_precision/HHS_mixed.dat};
            \addlegendentry{mixed}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vx,
            ymin=-40,
            ymax=40,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vy,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vy,x=t]{figures/adaptive_precision/HHS_mixed.dat};
            \addlegendentry{mixed}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}[b]{0.55\textwidth}
    \begin{tikzpicture}
        \begin{axis}[
            xlabel=time,
            ylabel=vz,
            ymin=-40,
            ymax=40,
            enlargelimits = false
           ]
            \addplot[black,thin] table [y=vz,x=t]{figures/adaptive_precision/HHS_ref.dat};
            \addplot[red,thin] table [y=vz,x=t]{figures/adaptive_precision/HHS_mixed.dat};
            \addlegendentry{mixed}
            \addlegendentry{reference}
        \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \caption{TODO, but this is mixed}
\end{figure}

==> figures/analytical_scenarios/lagrange_sin_approximation.tex <==

% orders 2, 4, 6
\begin{tikzpicture}{}
    \begin{axis}[
        xlabel=x,
        ylabel=sin($\pi x$),
        % enlargelimits = true,
        legend pos= north west
    ]
        \addplot[domain=-1:1, samples=20] function {sin(pi*x)};
        \addlegendentry{sin($\pi x$)}

        \addplot[blue, domain=-1:1, samples=20] function {
        0.839676613254*x
        % (2168036618656451 / 2581990000000000)*x
        };
        \addlegendentry{order 2}]

        \addplot[red, domain=-1:1, samples=20] function {
        (- 37157374616616943606603/ 12960272888918022041319)*x^3 
        +(34666924127372289653309974021060783 / 12960272888918022041319000000000000)*x
        };
        \addlegendentry{order 4}]

        \addplot[green, domain=-1:1, samples=20] function {
            (3642903721708520506423762842398198663125000000000/2114508035381203055004787720376812570420310944263)*x^5
            - (81363185062717170162827285033163832365583779597005 / 16916064283049624440038301763014500563362487554104)*x^3
            + (24991240597300848034797156644172758224312372789207270831923 / 8055268706214106876208715125245000268267851216240000000000)*x
        };
        \addlegendentry{order 6}

        %adding dots to show interpolation points
        \addplot [blue, only marks] table {
            -0.774597 -0.6504109855969353
            0 0.0
            0.774597 0.6504109855969353
        };
        \addplot [red, only marks] table {
            -0.906180 -0.29049539817270026
            -0.538469 -0.9927059291652813
            0 0.0
            0.538469 0.9927059291652813
            0.906180 0.29049539817270026
        };
        \addplot [green, only marks] table {
            -0.949108 -0.15920200241934077
            -0.741531 -0.7256673994165866
            -0.405845 -0.9565703703250715
            0 0.0
            0.405845 0.9565703703250715
            0.741531 0.7256673994165866
            0.949108 0.15920200241934077
        };
    \end{axis}
\end{tikzpicture}


% orders 3, 5
% \begin{tikzpicture}{}
%     \begin{axis}[
%         xlabel=x,
%         ylabel=sin($\pi x$),
%         % enlargelimits = true,
%         legend pos= north west
%     ]
%         \addplot[domain=-1:1, samples=20] function {sin(pi*x)};
%         \addlegendentry{sin($\pi x$)}]
        
%         \addplot[red, domain=-1:1, samples=20] function {
%         (-10182278524854636829545 / 3054410222531913594436) *x^3 
%         +(1809894976580170007579262553193949 / 610882044506382718887200000000000)*x                
%         };
%         \addlegendentry{order 3}]

%         \addplot[blue, domain=-1:1, samples=20] function {
%         (9412424961315549518515420708378622717500000000 / 5117609372027690649823734319421202687079015083) *x^5
%         - (95404473197347039149490435402753451948971209559 / 19311733479349776037070695544985670517279302200) *x^3
%         + (712106717005320109587318155443081759487332240961897416478863 / 227449305423452917769943747529831230536845114800000000000000)*x
%         };
%         \addlegendentry{order 5}
        
%         \addplot [red, only marks] table {
%             -0.861136 -0.4225464922307973
%             -0.339981 -0.876277951991784
%             0.339981   0.876277951991784
%             0.861136   0.4225464922307973
%         };
%         \addplot [blue, only marks] table {
%             -0.932469 -0.21056547042961016
%             -0.661209 -0.8744700481838902
%             -0.238619 -0.6813784246455376
%             0.238619   0.6813784246455376
%             0.661209   0.8744700481838902
%             0.932469   0.21056547042961016
%         };
%     \end{axis}
% \end{tikzpicture}

==> figures/analytical_scenarios/planar_wave.tex <==
% \begin{tikzpicture}
%     \begin{axis}
%         \addplot3[domain=-1:1, samples=100, samples y=100] function {cos(-pi*(x+y))};
%     \end{axis}
% \end{tikzpicture}
\begin{tikzpicture}{}
    \begin{axis}
        \addplot3[surf, domain=-1:1, samples=20, samples y=20] function {cos(-pi*(x+y))};%{0.02*(1+exp(-0.5*(x*x+y*y)/0.01))};
    \end{axis}
\end{tikzpicture}

==> figures/convergence/elastic_comparison_14_10/elastic.tex <==
\definecolor{lightGreen}{rgb}{.2,.8,.6}

\begin{figure}
    \centering
    \scalebox{.85}{\begin{tikzpicture}[font=\LARGE]
        \begin{semilogyaxis}[
            xlabel=polynomial order,
            ylabel=l2 error,
            enlargelimits = true,
            xtick=data
           ]
            \addplot[lightGreen,thick,mark=otimes*] table [y=l2,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_2.dat};
            \addlegendentry{l2, 9x9 cells}
            \addplot[teal,thick,mark=otimes*] table [y=l2,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_3.dat};
            \addlegendentry{l2, 27x27 cells}
        \end{semilogyaxis}
    \end{tikzpicture}}
    \scalebox{.85}{\begin{tikzpicture}[font=\LARGE]
        \begin{semilogyaxis}[
            xlabel=polynomial order,
            ylabel=$l_\infty$ error,
            enlargelimits = true,
            xtick=data
           ]
            \addplot[purple,thick,mark=otimes*] table [y=max,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_2.dat};
            \addlegendentry{$l_\infty$, 9x9 cells}
            \addplot[violet,thick,mark=otimes*] table [y=max,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_3.dat};
            \addlegendentry{$l_\infty$, 27x27 cells}]
        \end{semilogyaxis}
    \end{tikzpicture}}
    \scalebox{0.85}{\begin{tikzpicture}[font=\LARGE]
        \begin{semilogyaxis}[
            xlabel=polynomial order,
            ylabel=vx error,
            enlargelimits = true,
            xtick=data
           ]
            \addplot[cyan,thick,mark=otimes*] table [y=vx,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_2.dat};
            \addlegendentry{\Large{vx, 9x9 cells}}
            \addplot[blue,thick,mark=otimes*] table [y=vx,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_3.dat};
            \addlegendentry{\Large{vx, 27x27 cells}}]
        \end{semilogyaxis}
    \end{tikzpicture}}
    \scalebox{0.85}{\begin{tikzpicture}[font=\LARGE]
        \begin{semilogyaxis}[
            xlabel=polynomial order,
            ylabel=l2 interpolated error,
            enlargelimits = true,
            xtick=data
           ]
            \addplot[olive,thick,mark=otimes*] table [y=l2_interpolated,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_2.dat};
            \addlegendentry{\large{l2 interpolated, 9x9 cells}}
            \addplot[brown,thick,mark=otimes*] table [y=l2_interpolated,x=Order]{figures/convergence/elastic_comparison_14_10/elastic_depth_3.dat};
            \addlegendentry{\large{l2 interpolated, 27x27 cells}}]
        \end{semilogyaxis}
    \end{tikzpicture}}
    \caption{Elastic planar waves, alles fp32, unterschiedliche Messungen von dem Fehler.}
    \label{fig:comparison_errors_elastic}
\end{figure}

==> figures/initial_errors/table_initial_errors.tex <==
\begin{table}[!ht]
    \begin{adjustwidth}{-1.5cm}{}
    \begin{tabular}{ |c| c|| c|c|c|c| c|c|c|c| } 

        \hline
            & &
            \multicolumn{4}{|c|}{Elastic planar waves} & \multicolumn{4}{|c|}{Euler gaussian bell} \\
        \hline
        mesh depth & polynomial order & bf16 & fp16 & fp32 & fp64 & bf16 & fp16 & fp32 & fp64 \\
        \hline

         & 3 & $4.62e^{-02}$ & \texttt{NAN} & $3.38e^{-04}$ & $3.38e^{-04}$ & $1.20e^{-02}$ & $1.25e^{-03}$ & $3.86e^{-06}$ & $3.84e^{-06}$\\

        2 & 5 & $3.59e^{-02}$ & \texttt{NAN} & $7.68e^{-07}$ & $2.91e^{-07}$ & $7.96e^{-03}$ & $1.49e^{-03}$ & $2.06e^{-07}$ & $5.53e^{-08}$ \\
        
         & 7 & $3.61e^{-02}$ & \texttt{NAN} & $5.74e^{-07}$ & $1.51e^{-10}$ & $8.87e^{-03}$ & $1.80e^{-03}$ & $1.95e^{-07}$ & $6.12e^{-10}$ \\

        \hline

         & 3 & $1.39e^{01}$ & \texttt{NAN} & $1.59e^{-07}$ & $1.36e^{-07}$ & $1.23e^{-02}$ & $8.75e^{-04}$ & $1.89e^{-07}$ & $2.06e^{-08}$ \\

        3 & 5 & $1.39e^{01}$ & \texttt{NAN} & $5.72e^{-09}$ & $3.50e^{-15}$ & $1.53e^{-03}$ & $7.90e^{-03}$ & $1.98e^{-07}$ & $2.98e^{-11}$ \\
        
         & 7 & $5.12e^{01}$ & \texttt{NAN} & $1.03e^{-08}$ & $2.38e^{-23}$ & $1.83e^{-03}$ & $8.95e^{-03}$ & $1.88e^{-07}$ & $3.50e^{-12}$ \\

        \hline
    \end{tabular}
    \caption{\label{table:initial_errors_per_precision} TODO}
    \end{adjustwidth}
\end{table}
